Menger Curve and Non-Planar Boundaries in Quotients of Hyperbolic Groups

We study the persistence of non-planarity in boundaries of hyperbolic groups under quotients, focusing on quotients by large enough powers of infinite order elements. We prove that the non-planarity of the boundary of a one-ended hyperbolic group is preserved under such quotients. As a consequence, we obtain an analogous result about the persistence of Menger curve boundaries.

==> Figures/menger0.tex <==
\fill[menger2] (1, 1, 1) -- (1, -1, 1) -- (-1, -1, 1) -- (-1, 1, 1) -- cycle;
\fill[myblue] (1, 1, 1) -- (1, 1, -1) -- (1, -1, -1) -- (1, -1, 1) -- cycle;
\fill[mypurple] (1, 1, 1) -- (1, 1, -1) -- (-1, 1, -1) -- (-1, 1, 1) -- cycle;

==> Figures/menger1.tex <==
\begin{scope}[scale=.3333333333]
\begin{scope}[shift={(-2, -2, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(0, -2, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, -2, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, 0, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, 0, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, 2, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(0, 2, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, 2, -2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, -2, 0)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, -2, 0)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, 2, 0)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, 2, 0)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, -2, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(0, -2, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, -2, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, 0, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, 0, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(-2, 2, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(0, 2, 2)}]
\input{Figures/menger0}
\end{scope}
\begin{scope}[shift={(2, 2, 2)}]
\input{Figures/menger0}
\end{scope}
\end{scope}
